Make The Most of Prior Data: A Solution for Interactive Text Summarization with Preference Feedback

For summarization, human preference is critical to tame outputs of the summarizer in favor of human interests, as ground-truth summaries are scarce and ambiguous. Practical settings require dynamic exchanges between human and AI agent wherein feedback is provided in an online manner, a few at a time. In this paper, we introduce a new framework to train summarization models with preference feedback interactively. By properly leveraging offline data and a novel reward model, we improve the performance regarding ROUGE scores and sample-efficiency. Our experiments on three various datasets confirm the benefit of the proposed framework in active, few-shot and online settings of preference learning.

==> intro.tex <==
% Human-In-The-Loop:

% - Online learning 

% - Interactive learning

%     -- Active learning
    
%     --- Bayesian Optimization
    
%     --- Online RL:
    
%         ------ Absolute reward
        
%         ------ OUR: Relative reward -- Human preference

 The advent of Artificial Intelligence (AI) has changed business practices. The human roles in interaction with AI-powered machines have been evolving and the new human roles are explicit in the concept of human-in-the-loop (HITL). (HITL) allows human to actively participate in supervising AI systems; reject or approve or label outputs of the machines, or provide expert-advice to the machines as the unique source of external knowledge. By observing the outcomes of AI systems, human can embrace some potential outcomes and then can feed back for retraining and fine tuning the AI models. It will arguably turn down the runtime and memory consumption and make the outputs more explainable to the user. (HITL) can make AI-powered machines more commercially viable for businesses. [Wu, et. al. 2021] argued that adding priori knowledge through (HITL) to deep learning models would slash the operating cost as the models won't need to consume extra computing power extracting knowledge from the training data. The other opportunity they argued is that the model learning-performance would benefit from (HITL) where collecting eanough training data could be impossible or expensive or the solution spaces are too large [Icarte, et. al.,2018] to search for optimal solutions. That is true where the user deals with real-time data, or when the context changes, or where the user's preference matters. Some NLP tasks; e.g. documents summarization is a good candidate where the ultimate gold-standard summaries for labeling are either multifaceted (human-preference) or do not exist [Simpson, Gurevych, 2018]. In such casea, (HITL) can positively impact the performance of NLP summarization task and can determine the quality of the outputs. 
There is a growing research body of (HITL) NLP frameworks,  where model developers continuously integrate human feedback into different steps of the model deployment workflow. Abstractive  document summarization is indeed a subjective task [Stiennon, et al. 2020] and hard to quantify what makes a “good summary” without human judgment input. However, in previous methods collecting human feedback and evaluation of the crafted summaries from documents had been done during building the training datasets. That is time-consuming [Wu et. al., 2021] and expensive particularly where the domain-knowledge is required. Uc-Cetina, et. al., [2021] argue the importance of the user’s intentions for modeling Natural Language Understanding with high performance. The authors considered that the nature of the user’s intentions was diverse and uncertain, while that nature was sequential and context-specific. So, given these attributions, the reinforcement learning (RL) paradigm is an appropriate choice for modeling the user’s internal semantic representations. 
To address that challenge, we deployed (HITL) along with the (RL) approach in our text summarization framework to continuously collect the user-feedback and consequently improve model prediction robustness. 

To formulate NLP document summarization tasks with HITL, we define the text summarization tasks as the process of distilling the most relevant information from source documents to construct a shortened version for particular users [Mani, 1999] while imitating human-like summarization [Fiori 2014]. In this definition, the user’s intention is implicitly acknowledged as a factor that influences the extraction of information from the source documents. Upon this definition, we shall architect summarization algorithms that not only will be trained with human-produced summaries datasets but the model will be also adapted as more human-feedback is fed in.
We acknowledge the key challenges in architecting such an algorithm that would be commercially feasible. Convergence to an optimal set of summaries using only reinforcement learning requires accumulating a substantial volume of preferences from each user. This is an expensive approach as collecting preferences practically takes huge human-resources. Previous studies collected human-feedback-judgments and aggregating binary votes from multiples human-raters (Wei et al., 2016). However, the cost of hiring human-raters puts a limitation on this sort of output-rating approach (Persing and Ng, 2017). To minimize the use's effort to provide feedback for training a ranker, [Wirth et al., 2017] proposed an RL agent that could find the optimal solution. Active learning along with (RL) can be an option to tackle the above mentioned challenge. [Gao et al. 2018] introduced such a model with an acquisition function which was minimized for the number of interaction. However, these approaches are not yet efficient as they rank entite the solution space including relevant and irrelevant pairs which is waste of computing power. In effect, most business users just need to rank a small set of relevant candidates. It sounds like Bayesian optimization (BO) could be an appropriate alternative to address the above shortcoming of the interactive method for ranking texts. [Siddhant and Lipton, 2018;Peris and Casacuberta, 2018] substituted the standard uncertainty- based acquisition functions in (AL) with more suitable functions for (BO). Their models minimized the number of feedback needed in order to get the optimum solutions. (BO) does not need to learn the entire ranking function, so, the irrelevant solutions are disregarded and the approach can potentially save computing power and time. However, (BO) with expected improvement (IMP) strategy approach and Thompson sampling (TP) still consumes a lot of computing power for a larger number of iterations. This could stem from the sparsity of sample solutions.
Another challenge is to what extent we can assure the human-summaries are reliable as preferences. 


% \textbf{[General Direction]} 
% \begin{itemize}
% \item Goal: It is to find the best solution from a large space of possible solutions to meet a particular user’s needs. A possible approach to small the size of the possible answers space and to consider human-preference is an interactive text ranking approach that actively selects pairs of candidates, from which the user selects the best.
% \item Strategies: Any sort of machine learning approach that can rank the pair of {query, possible answer} across the whole candidate space and also it must be interactive to bring in human’s feedbacks. A good strategy should have a clear understanding of the whole topic and the user’s intention as Agichtein argued [2008]. 
% \item Characteristics: (1) interactive to efficiently gather user feedbacks (2) capability to combine the user feedbacks with predictions from pretrained, (3) capable to be adaptable, scalable and being a generic model.. 
% \end{itemize}

% \textbf{[The Challenges]}:
% \begin{itemize}
% \item It is hard if not impossible or expensive to find enough task-specific training data 
% \item user’s intentions - value judgments - preference varies significantly and they are all context-specific \item to be practical, sample-efficiency in terms of number of interactions is a must. 
% \end{itemize}

% \textbf{[Issues with prior HITL for NLP]}
% \begin{itemize}
%   \item Online learning: RL approach, supervised apprach,etc. Preference Learning: a good approach in order to minimize the amount of effort the user needs to expend to train a ranker and use an RL agent to find the optimal solution [Wirth et al., 2017]
%   \item Active learning: BO, Dropout-uncertainty, etc. Active Learning: a good approach in order to reduce the number of labels a user needs to provide. It is a learning paradigm in which a model by iteratively acquiring labels and at each iteration, it trains a model on the labels collected, then uses an acquisition function to quantify the value of querying the user about a particular pair of candidates. The acquisition function implements one of many different strategies to minimize the number of interaction rounds [PL + AL by Gao et al. 2018] . 
% Notes, These approaches rank all important/relevant and unimportant/irrelevant pairs which is unnecessary and wasting time and computing power. We usually just need to rank a small set of relevant candidates to present to the users.
% Bayesian Optimization: to address the above shortcoming of the interactive method for ranking texts the researchers replace the standard uncertainty- based acquisition functions in AL with acquisition functions for Bayesian optimization (BO). The objective of BO is to minimize the number of labels/feedback needed to find the best candidate, in contrast to uncertainty-based strategies that attempt to learn the entire ranking function. Thus, BO is a better approach to the summarization task where we want to find the best candidate and those with low quality can simply be disregarded rather than ranked precisely [Siddhant & Lipton, 2018;Peris & Casacuberta, 2018] 
% Notes: The previous research shows between two proposed Bayesian optimization strategies expected improvement (IMP) outperforms Thompson sampling (TP) where the goal is to optimize the proposed best solution. TP may require a larger number of interactions due to its random sampling step. IMP is effective in summarization tasks, but it requires a huge number of interactions. This may be due to the sparsity of candidates.
% \end{itemize}

Our contribution is three-fold:
\begin{itemize}
\item We propose new RL-based preference learning mechanisms for summarization task using novel sampling techniques on offline data
\item We show that our interactive preference learning with offline data can be applied to both online, active and few-shot learning scenerios
\item We conduct extensive empirical studies on 3 summarization datasets, showing that our proposed method outperform SOTA baselines regarding performance and sample-efficiency. 
\end{itemize}
